Third-Party Language Model Performance Prediction from Instruction

Language model-based instruction-following systems have lately shown increasing performance on many benchmark tasks, demonstrating the capability of adapting to a broad variety of instructions. However, such systems are often not designed to be transparent about their limitations; a user may easily prompt a model with an instruction without any idea of whether the responses should be expected to be accurate, or if the system is even capable of performing the task. We propose a third party performance prediction framework, where a separate model is trained to predict the metric resulting from evaluating an instruction-following system on a task while assuming access only to its inputs and outputs at inference time. We perform this analysis with a variety of both open and closed instruction-following models as well as multiple performance predictors, and examine the effect of various factors such as model size, number of training tasks, and prompt format. Our findings indicate that third-party performance prediction is very challenging, and much work remains in developing predictors that can automatically reveal the limitations of modern instruction-following natural language processing systems.

==> intro.tex <==
\section{Introduction}

Widespread modern efforts have aimed to develop language models (LMs) that serve as multipurpose tools by building models that can perform tasks simply by following natural language instructions. A large amount of recent work has explored this functionality with great success, by directly prompting pretrained models, performing additional maximum likelihood fine-tuning using curated instruction datasets for supervision, or improving performance even further with post-hoc procedures like RLHF to better align instruction-following behavior with human preferences.

A common goal of building an instruction-following model is having the model adapt to arbitrary instructions that were not seen at training time, i.e., cross-task generalization. Typically, cross-task generalization is assessed by evaluating the model on a suite of various tasks chosen to be sufficiently dissimilar from any tasks seen during instruction-tuning. This often involves using a human-annotated set of labeled instances for each evaluation task, with a number of benchmark datasets formatted in this way. Existing work examines the effect of various aspects of the model and training setup on cross-task generalization, including model size, number and diversity of tasks, and prompt format, among other factors.

However, it is important to understand how a model might generalize to a new task or instruction without simply running inference on a manually-curated evaluation set. Models that are made available to a wide range of users may be prompted with novel instructions that bear no similarity to those in benchmark datasets, with no existing evaluation data to determine whether or not the model can adequately perform the task. Predicting how well a model might respond to a novel task is crucial for appropriately handling cases where the model cannot perform the task adequately, either by warning a user to use the output with caution, declining to perform tasks that the model cannot confidently do, or routing certain tasks to a more competent model. Recent work attempts to address this issue by prompting or fine-tuning models to predict whether or not they can produce the correct output for individual task instances, typically drawn from factoid question answering or mathematical problem solving datasets. However, these limited use cases do not cover the broad range of possible ways in which a user might prompt a model to follow an instruction.

In this work, we examine whether model behavior can be predicted at the task level, by assessing whether or not we can predict an instruction-tuned model's performance given an instruction alone, using the model's known behavior on an existing set of instructions that it did not observe during training. \rahul{Feels like this ``main goal'' statement should come up much earlier in the intro, should find a way to move it to a previous paragraph.} We do so by training a regression model to predict some quantitative measure of model performance given a task instruction, and examine how predictability varies as a function of instruction-tuned model size, choice of instruction-tuning dataset, choice of evaluation metric to predict, and other factors. We find that while the choice of instruction-tuning dataset affects predictability and larger models are more predictable, the task of predicting model behavior from instructions given past performance remains challenging. Our works opens up the possibility of future attempts to predict how well a model will perform on a task given the task's instruction, an especially relevant goal as instruction-following models continue to become more widely adopted.

\rahul{Lots of previous work to mention above, need to go through this section carefully and add the relevant citations.}

\begin{comment}

\begin{itemize}

    \item Much recent work explores prompting language models to perform tasks by following instructions

    \begin{itemize}
    
        \item Includes models solely trained as language models (GPT-3, LLaMA), fine-tuned with supervision to follow instructions (T0, FLAN, Tk-Instruct, Alpaca, Vicuna, Tülu), or fine-tuned and then updated with post-hoc procedures like RLHF (InstructGPT, ChatGPT)
        
    \end{itemize}

    \item A common goal of this work is building models that can follow arbitrary instructions, i.e., cross-task generalization

    \begin{itemize}

        \item Existing work (T0, FLAN, Tk-Instruct) examines cross-task generalization capabilities as a function of various aspects of training (number of tasks, number of instructions per task, model size, etc.)

        \item Some claim that signs of true generalization to unseen instructions already exists (``Sparks of AGI'' paper)

    \end{itemize}

    \item Massive datasets exist to assess cross-task generalization (Super-NaturalInstructions, Self-Instruct, FLAN v2, MMLU, BIG-Bench, others), typically with evaluation instances for each task in a held-out set

    \item However, it's important to understand how a model might generalize to a new task/instruction without simply running inference on an evaluation set
    
    \begin{itemize}

        \item Models ``in the wild'' might see completely novel instructions from users with no similarity to instructions from benchmark datasets and no existing evaluation data
        
    \end{itemize}

    \item One avenue for attempting to assess cross-task generalization without evaluation is by predicting model performance from task instruction alone, either by prompting the model (not a focus of this work) or training a separate performance prediction model

    \item Recent work performs this kind of assessment at the instance level (e.g., ``Language Models (Mostly) Know What They Know'', others -- see Sec.~\ref{sec:related}) by either prompting or fine-tuning the original model, but this generally assesses factual knowledge or specific skills (math problem solving, code generation) and not generalization to arbitrary tasks from instruction

    \item This work proposes various methods for predicting whether a model might generalize to unseen tasks/instructions, and performs analyses to assess which factors lead to better predictability of model performance
    
\end{itemize}

\end{comment}

==> todo.tex <==
{
\color{red}
\section*{To-do}

\begin{itemize}

    \item Lots of recent work prompts the model directly to emit its confidence either through logits (``True/False'' probability) or verbalized confidence (``I am 90\% confident...'') -- might be worth doing this analysis on instruction-tuned LLaMA models as well

    \item Use consistent performance predictor model (most experiments use RoBERTa-large, but some only use RoBERTa-base)

    \item Make sure decisions that were made early and fixed are still valid -- random split by task? ROUGE-L as the metric to predict (for most experiments)?

    \item Run experiments on larger LLaMA model sizes to assess effect of model scale (currently only using 7B-parameter model)

    \item Run experiments using base LLaMA model as performance predictor model as well, to see effect of instruction-tuning on being able to predict performance

\end{itemize}
}
